Enabling Small Models for Zero-Shot Selection and Reuse through Model Label Learning

Vision-language models (VLMs) like CLIP have demonstrated impressive zero-shot ability in image classification tasks by aligning text and images but suffer inferior performance compared with task-specific expert models. On the contrary, expert models excel in their specialized domains but lack zero-shot ability for new tasks. How to obtain both the high performance of expert models and zero-shot ability is an important research direction. In this paper, we attempt to demonstrate that by constructing a model hub and aligning models with their functionalities using model labels, new tasks can be solved in a zero-shot manner by effectively selecting and reusing models in the hub. We introduce a novel paradigm, Model Label Learning (MLL), which bridges the gap between models and their functionalities through a Semantic Directed Acyclic Graph (SDAG) and leverages an algorithm, Classification Head Combination Optimization (CHCO), to select capable models for new tasks. Compared with the foundation model paradigm, it is less costly and more scalable, i.e., the zero-shot ability grows with the sizes of the model hub. Experiments on seven real-world datasets validate the effectiveness and efficiency of MLL, demonstrating that expert models can be effectively reused for zero-shot tasks. Our code will be released publicly.

==> sections/algorithms/algorithm1.tex <==
\begin{algorithm}[t!]
\caption{Classification
Head Combination Optimization (CHCO) Algorithm}
\label{alg:alg1}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} model label \(S\), match class space \(\mathcal{Y}'\), learning rate \(lr\), iterations \(n_{iter}\).
    \STATE \textbf{Output:} head combination variable \(\{\textbf{x}_c\}\) and loss \(\mathcal{L}_c\).
    \STATE Uniformly initialize \(X\).
    \STATE Calculate head-class probability matrix \(P\).
    \WHILE{not coverage or not reach \(n_{iter}\)}
        \FOR{\(h \in H_m\)}
            \STATE Fix \(\textbf{x}_{h'}\) for other heads and calc. gradient for \(\textbf{x}_{h}\).
            \STATE Update \(\textbf{x}_{h}=\textbf{x}_{h}-lr\cdot \nabla_{\textbf{x}_h}\mathcal{L}\).
            \STATE Project \(\textbf{x}_h\) into the simplex.
        \ENDFOR
    \ENDWHILE
    \STATE Split \(X\) to \(|\mathcal{Y}'|\) head comb. \(\{\textbf{x}_c\}\) (expert predictors).
    \STATE Calculate loss \(\mathcal{L}_c\) on each class.
    \RETURN \(\{\textbf{x}_c\}, \mathcal{L}_c\)
\end{algorithmic}
\end{algorithm}
